The communication cost of security and privacy in federated frequency estimation

We consider the federated frequency estimation problem, where each user holds a private item $X_i$ from a size-$d$ domain and a server aims to estimate the empirical frequency (i.e., histogram) of $n$ items with $n \ll d$. Without any security and privacy considerations, each user can communicate its item to the server by using $\log d$ bits. A naive application of secure aggregation protocols would, however, require $d\log n$ bits per user. Can we reduce the communication needed for secure aggregation, and does security come with a fundamental cost in communication? In this paper, we develop an information-theoretic model for secure aggregation that allows us to characterize the fundamental cost of security and privacy in terms of communication. We show that with security (and without privacy) $\Omega\left( n \log d \right)$ bits per user are necessary and sufficient to allow the server to compute the frequency distribution. This is significantly smaller than the $d\log n$ bits per user needed by the naive scheme, but significantly higher than the $\log d$ bits per user needed without security. To achieve differential privacy, we construct a linear scheme based on a noisy sketch which locally perturbs the data and does not require a trusted server (a.k.a. distributed differential privacy). We analyze this scheme under $\ell_2$ and $\ell_\infty$ loss. By using our information-theoretic framework, we show that the scheme achieves the optimal accuracy-privacy trade-off with optimal communication cost, while matching the performance in the centralized case where data is stored in the central server.

==> sec_dropout.tex <==

In this section, we give details on how to extend our framework to tolerate a fraction of dropout users $\mathcal{D} \subset [n]$.  In order to do this, we need to develop a  characterization (i.e., an information-theoretic model) of secure aggregation schemes that can tolerate up to $d$ dropouts and can potentially handle colluding users or a honest-but-curious server.  %We start with a simple model and then extend it to include a larger set of schemes which can potentially handle colluding users or a honest-but-curious server.

We define a secure aggregation scheme that can tolerate up to $d$ dropouts as consisting of two stages: 
\begin{enumerate}
\item Users send their messages $Y_i$ as in Figure~1;
\item Server invokes a second round of communication with the surviving clients to recover the masks of the dropout users. In this round, the server collects $g\left( \theta_{[n]}, \mathcal{D} \right)$, where $g(\cdot)$ is a general function of local secrets $\theta_{[n]}$ such that (1) if $|\mathcal{D}| \leq d$, the masks of the dropout users can be recovered correctly; (2) if $|\mathcal{D}|>d$, no information is leaked to the server.
\end{enumerate}  
Formally, the secure constraints (S1) and (S2) in the original version are modified as follows:
\begin{align}
    &\forall \mathcal{D} \subseteq [n],\, I\left( Y_{[n]\setminus \mathcal{D}}, g\left( \theta_{[n]}, \mathcal{D} \right); X_{[n]} \middle\vert \mu\left( X_{[n]\setminus \mathcal{D}} \right)\right) = 0 \tag{S1'}\label{S1'}, \\
     & \forall |\mathcal{D}| > d, \, I\left( Y_{[n]\setminus \mathcal{D}}, g\left( \theta_{[n]}, \mathcal{D} \right); X_{[n]} \right) = 0. \tag{S2'}\label{S2'}
\end{align}
(S1') ensures the server can only learn the sum of the participating clients; (S2') requires that $g(\cdot)$ is designed in a way that when the masks cannot be recovered, which is the case when $|\mathcal{D}|> d$, no information from $\left(  Y_{[n]\setminus \mathcal{D}}, g\left( \theta_{[n]}, \mathcal{D} \right) \right)$ is revealed to the server. 

In addition, with dropout, one can no longer hope to recover the sum (or the approximate sum) for all clients, and hence the correctness conditions (C1) and (C1$^\prime$) are replaced with
\begin{align}
    &\forall |\mathcal{D}| \leq d,\,\Pr\left\{ f\left( Y_{[n]\setminus \mathcal{D}}, g\left( \theta_{[n]}, \mathcal{D} \right) \right) =  \mu\left( X_{[n]\setminus \mathcal{D}} \right) \right\} = 1, \text{ and }
\tag{C2}\label{C2}\\
    & \forall |\mathcal{D}| \leq d,\,\mathbb{E}\left[ \ell \left( f\left( Y_{[n]\setminus \mathcal{D}}, g\left( \theta_{[n]}, \mathcal{D} \right) \right),  \mu\left( X_{[n]\setminus \mathcal{D}} \right)\right) \right] \leq \beta.\tag{C2'}\label{C2prime}
\end{align}
We note that the extension of SecAgg to handle dropouts in [Bonawitz et. al 2017] falls in this class.

Next, we show that under the modified constraints, our communication lower bounds still hold, except for replacing $n$ with $n-\left\lvert\mathcal{D}\right\rvert$ in all previous lower bounds. At a high level, it suggests that \emph{for any scheme of the form above that allows for dropouts, the best communication cost one can hope for is the same as running the original protocol on the remaining $n-|\mathcal{D}|$ users.} %Intuitively, handling dropouts only makes the problem ``harder'', and hence the communication complexity can only increase (or at least remains the same). 


Now, under the new constraints, we state and prove lower bounds analogous to Lemma~3.1 and Lemma~3.2. Note that at a high level, the only modification is to view 
$ \left( Y_{[n]\setminus \mathcal{D}}, g\left( \theta_{[n]}, \mathcal{D} \right) \right) $ as a new variable $\tilde{Y}_{[n]\setminus \mathcal{D}}$, and the rest of the proof follows.

\begin{lemma}[Lower bound for perfect recovery]\label{lemma::noiseless_dropout_lower_bound}
Let $\mathcal{D} \subset [n]$ be the set of dropout clients, such that $\mathcal{D} \leq d$ for some $d \leq \frac{n}{2}$. Under the correctness constraint (C2) and security constraints (S1') and (S2'), it holds that for all $i \in [n]\setminus\mathcal{D}$, $H(Y_i) \geq H\left( \sum_{i\in[n]\setminus \mathcal{D}} X_i \right),$
where $H(\cdot)$ is the Shannon entropy.
\end{lemma}
\begin{proof}
First of all, observe that for any $\mathcal{D} \subset [n]$ such that $\mathcal{D} \leq d$
\begin{align*}
    & I\left( X_{[n]}; Y_{[n]\setminus \mathcal{D}}, g\left( \theta_{[n]}, \mathcal{D} \right) \right) \\
    &= I\left( \sum_{i\in [n]\setminus \mathcal{D}} X_i; Y_{[n]\setminus \mathcal{D}}, g\left( \theta_{[n]}, \mathcal{D} \right)\right) + I\left( Y_{[n]\setminus \mathcal{D}}, g\left( \theta_{[n]}, \mathcal{D} \right); X_{[n]} \middle\vert \sum_{i \in [n]\setminus \mathcal{D}} X_i \right) \\
    & = I\left( \sum_{i\in [n]\setminus \mathcal{D}} X_i; Y_{[n]\setminus \mathcal{D}}, g\left( \theta_{[n]}, \mathcal{D} \right)\right) \\
    & = H\left( \sum_{i\in [n]\setminus \mathcal{D}}  X_i\right) - H\left( \sum_{i\in [n]\setminus \mathcal{D}}  X_i \middle\vert Y_{[n]\setminus \mathcal{D}}, g\left( \theta_{[n]}, \mathcal{D} \right)\right)\\
    & = H\left( \sum_{i\in [n]\setminus \mathcal{D}}  X_i\right),
\end{align*}
where the second equality holds due to (S1') and the third equality holds since (C2) implies $$H\left( \sum_{i\in [n]\setminus \mathcal{D}}  X_i \middle\vert Y_{[n]\setminus \mathcal{D}}, g\left( \theta_{[n]}, \mathcal{D} \right)\right) = 0. $$ On the other hand, let $\mathcal{D'} \subset [n]$ be such that $|\mathcal{D'}| = d$ and let $j \in \mathcal{D}\setminus j$ we also have
\begin{align}\label{eq:lossless_mi_upperbound_dropout}
    &I\left( X_{[n]}; Y_{[n]\setminus \mathcal{D'}}, \theta_{\mathcal{D}'} \right) \nonumber\\ 
    &= I\left(  Y_{[n]\setminus \left\{ \{j\} \vee \mathcal{D'}\right\}}, \theta_{\mathcal{D'}\vee \{j\}} ; X_{[n]} \right) + I\left(  Y_{j} ; X_{[n]} \middle\vert Y_{[n]\setminus \left\{ \{j\} \vee \mathcal{D'}\right\}}, \theta_{\mathcal{D'}\vee \{j\}}  \right) \nonumber\\
    &= I\left(  Y_{j} ; X_{[n]} \middle\vert Y_{[n]\setminus \left\{ \{j\} \vee \mathcal{D'}\right\}}, \theta_{\mathcal{D'}\vee \{j\}}  \right) \nonumber \\
    &= H\left(  Y_{j} \middle\vert Y_{[n]\setminus \left\{ \{j\} \vee \mathcal{D'}\right\}}, \theta_{\mathcal{D'}\vee \{j\}} \right) -  H\left(  Y_{j} \middle\vert Y_{[n]\setminus \left\{ \{j\} \vee \mathcal{D'}\right\}}, \theta_{\mathcal{D'}\vee \{j\}}, X_{[n]} \right) \nonumber\\
    & \leq H\left(  Y_{j} \middle\vert Y_{[n]\setminus \left\{ \{j\} \vee \mathcal{D'}\right\}}, \theta_{\mathcal{D'}\vee \{j\}} \right) \nonumber\\
    & \leq H\left(  Y_{j} \right),
\end{align}
where the second equality is due to \eqref{S2'}. %\qedwhite
\end{proof}


\begin{lemma}\label{lemma:lossy_dropout_lower_bound}
Let $\ell(\cdot, \cdot)$ be a loss function defined on the domain of $ \mu\left( X^{n-|\mathcal{D}|} \right) = \sum_{i\in[n]\setminus \mathcal{D}} X_i$. Under the $\beta$-approximate recovery criterion \eqref{C2prime} and the security constraints \eqref{S1'} and \eqref{S2'}, it holds that 
$$ H(Y_i) \geq R(\beta) \text{, for all } i \in [n],$$
where $R(\beta)$ is the solution of the following rate-distortion problem:
\begin{equation}\label{eq:rate_function}
R\left( \beta \right) := 
    \begin{pmatrix}
    & \min_{P_{Y^{n'} |\mu\left( X^{n'} \right)}} & I\left( Y^{n'} ;  \mu\left( X^{n'} \right)\right)\\
    & \textrm{subject to } &\min_{\hat{\mu}} \mathbb{E}\left[ \ell\left( \hat{\mu}\left( Y^{n'}  \right),  \mu\left( X^{n'} \right) \right) \right] \leq \beta,
    \end{pmatrix}
\end{equation}
where $n' := n - |\mathcal{D}|$.
\end{lemma}
\begin{proof}
Notice that by \eqref{eq:lossless_mi_upperbound_dropout}, we have $H(Y_i) \geq I\left( X_{[n]}; Y_{[n]\setminus\mathcal{D}}, g\left( \theta_{[n]}, \mathcal{D} \right) \right)$. Therefore, it suffices to lower bound $I\left( X_{[n]}; Y_{[n]\setminus\mathcal{D}}, g\left( \theta_{[n]}, \mathcal{D} \right) \right)$ subject to \eqref{C2prime}, \eqref{S1'}, and \eqref{S2'}. Using \eqref{S1'}, we have 
$$ I\left( X_{[n]}; Y_{[n]\setminus\mathcal{D}}, g\left( \theta_{[n]}, \mathcal{D} \right) \right) = I\left( \sum_{i\in[n]\setminus\mathcal{D}} X_i; Y_{[n]\setminus\mathcal{D}}, g\left( \theta_{[n]}, \mathcal{D} \right) \right) \geq I\left( \sum_{i\in[n]\setminus\mathcal{D}} X_i; Y_{[n]\setminus\mathcal{D}}\right).$$ 

Constrained on \eqref{C2prime}, this quantity is lower bounded by $R(\beta)$.
\end{proof}
